The particle spectra of parity-violating theories: A less radical approach and an upgrade of PSALTer

Due to computational barriers, the effects of parity violation have so far been grossly neglected in gravitational model-building, leading to a serious gap in the space of prior models. We present a new algorithm for efficiently computing the particle spectrum for any parity-violating tensorial field theory. It allows to extract conditions for the absence of massive ghosts without resorting to any manipulation of radicals in cases where the particle masses are irrational functions of the Lagrangian coupling coefficients. We test it against several examples, among which is the most general parity-indefinite Einstein-Cartan/Poincar\'e gravity that propagates two healthy massive scalars (in addition to the massless graviton). Importantly, we upgrade the PSALTer software in the Wolfram Language to accommodate parity-violating theories. PSALTer is a contribution to the xAct project.

==> MacrosMath.tex <==
%%======================%%
%%  Indexed quantities  %%
%%======================%%

\makeatletter
\newcommand{\dalembertian}{\mathop{\mathpalette\dalembertian@\relax}}
\newcommand{\dalembertian@}[2]{%
  \begingroup
  \sbox\z@{$\m@th#1\square$}%
  \dimen0=\fontdimen8
    \ifx#1\displaystyle\textfont\else
    \ifx#1\textstyle\textfont\else
    \ifx#1\scriptstyle\scriptfont\else
    \scriptscriptfont\fi\fi\fi3
  \makebox[\wd\z@]{%
    \hbox to \ht\z@{%
      \vrule width \dimen0
      \kern-\dimen0
      \vbox to \ht\z@{
        \hrule height \dimen0 width \ht\z@
        \vss
        \hrule height 2\dimen0
      }%
      \kern-2.5\dimen0
      \vrule width 2.5\dimen0
    }%
  }%
  \endgroup
}
\makeatother

\def\vect#1{\mbox{\boldmath $#1$}}

\newrobustcmd{\SmashAcute}[1]{%
	{\vphantom{#1}\smash{\Acute{#1}}}
}
\newrobustcmd{\MinimumPower}[1]{%
	{n_{#1}} 
}
\newrobustcmd{\ComponentTotal}{%
	{\mathsf{j}_{\text{T}}} 
}
\newrobustcmd{\ConstraintTotal}{%
	{\mathsf{v}_{\text{T}}} 
}
\newrobustcmd{\MPl}{%
	{M_{\mathrm{Pl}}} 
}
\newrobustcmd{\Coordinates}[1]{%
	{\tensor{x}{#1}}%
}
\newrobustcmd{\Momenta}[1]{%
	{\tensor{k}{#1}}%
}
\newrobustcmd{\IdentityJ}[1]{%
	{\mathsf{1}_{}}%
}
\newrobustcmd{\IdentityJP}[2]{%
	{\mathsf{1}_{{#1^#2}}}%
}
\newrobustcmd{\Jp}{%
	{J{'}}%
}
\newrobustcmd{\Pp}{%
	{P{'}}%
}
\newrobustcmd{\Ppp}{%
	{P{''}}%
}
\newrobustcmd{\Pppp}{%
	{P{'''}}%
}
\newrobustcmd{\Sp}{%
	{s{'}}%
}
\newrobustcmd{\Ap}{%
	{a{'}}%
}
\newrobustcmd{\Bp}{%
	{b{'}}%
}
\newrobustcmd{\Cp}{%
	{c{'}}%
}
\newrobustcmd{\GKPu}[1]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$1$}{\scriptsize$\tilde u$}\big)}}{#1}}%
}
\newrobustcmd{\GKPs}[1]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$0$}{\scriptsize$\tilde s$}\big)}}{#1}}%
}
\newrobustcmd{\GKP}[1]{%
	{\tensor{{{\mathscr{P}}^1_{v}}}{#1}}%
}
\newrobustcmd{\GKPv}[1]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$1$}{\scriptsize$v$}\big)}}{#1}}%
}
\newrobustcmd{\GKPvt}[1]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$1$}{\scriptsize$\tilde{v}$}\big)}}{#1}}%
}
\newrobustcmd{\GKPvtv}[1]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$1$}{\scriptsize$\tilde{v}v$}\big)}}{#1}}%
}
\newrobustcmd{\GKPvvt}[1]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$1$}{\scriptsize$v\tilde{v}$}\big)}}{#1}}%
}
\newrobustcmd{\GKPXX}[3]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$1$}{\scriptsize${#1}{#2}$}\big)}}{#3}}%
}
\newrobustcmd{\GKPX}[2]{%
	{\tensor{{{\mathscr{P}}\big(\stackanchor[1pt]{\scriptsize$1$}{\scriptsize${#1}$}\big)}}{#2}}%
}
\newrobustcmd{\ProjPara}[1]{%
	{\tensor*{\Theta}{#1}}%
}
\newrobustcmd{\kron}[1]{%
	{\tensor*{\delta}{#1}}%
}
\newrobustcmd{\metric}[1]{%
	{\tensor*{\eta}{#1}}%
}
\newrobustcmd{\ProjPerp}[1]{%
	{\tensor*{\Omega}{#1}}%
}
\newrobustcmd{\States}[4]{%
	{\tensor*{{#4}}{^{#3}_{{{#1}^{#2}}}}}%
}
\newrobustcmd{\FieldIndices}[2]{%
	{#2_#1}%
}
\newrobustcmd{\ParallelFieldIndices}[3]{%
	{{\overline{#3}}_{{#1^#2}}}%
}
\newrobustcmd{\FieldUp}[2]{%
	{\tensor{\zeta}{^{{\FieldIndices{#1}{#2}}}}}%
}
\newrobustcmd{\FieldUpTilde}[2]{%
	{\tensor{\tilde{\zeta}}{^{{\FieldIndices{#1}{#2}}}}}%
}
\newrobustcmd{\FieldDown}[2]{%
	{\tensor{\zeta}{_{\FieldIndices{#1}{#2}}}}%
}
\newrobustcmd{\FieldDownTilde}[2]{%
	{\tensor{\tilde{\zeta}}{_{\FieldIndices{#1}{#2}}}}%
}
\newrobustcmd{\FieldDownTildeConj}[2]{%
	{\tensor*{\tilde{\zeta}}{^*_{\FieldIndices{#1}{#2}}}}%
}
\newrobustcmd{\FieldDownConj}[2]{%
	{\tensor*{\zeta}{^*_{\FieldIndices{#1}{#2}}}}%
}
\newrobustcmd{\SourceUp}[2]{%
	{\tensor{j}{^{{\FieldIndices{#1}{#2}}}}}%
}
\newrobustcmd{\ConstrainedSourceUp}[2]{%
	{\tensor{\hat{j}}{^{{\FieldIndices{#1}{#2}}}}}%
}
\newrobustcmd{\SourceTildeUp}[2]{%
	{\tensor{\tilde{j}}{^{{\FieldIndices{#1}{#2}}}}}%
}
\newrobustcmd{\SourceTildeDown}[2]{%
	{\tensor{\tilde{j}}{_{{\FieldIndices{#1}{#2}}}}}%
}
\newrobustcmd{\SourceTildeDownConj}[2]{%
	{\tensor*{\tilde{j}}{^*_{{\FieldIndices{#1}{#2}}}}}%
}
\newrobustcmd{\SourceDown}[2]{%
	{\tensor{j}{_{\FieldIndices{#1}{#2}}}}%
}
\newrobustcmd{\SourceDownConj}[2]{%
	{\tensor*{j}{^*_{\FieldIndices{#1}{#2}}}}%
}
\newrobustcmd{\ConstrainedSourceDown}[2]{%
	{\tensor{\hat{j}}{_{\FieldIndices{#1}{#2}}}}%
}
\newrobustcmd{\FieldUpState}[5]{%
	{\tensor{\zeta\big(\States{#1}{#2}{#3}{#4}\big)}{^{{\ParallelFieldIndices{#1}{#2}{#5}}}}}%
}
\newrobustcmd{\SourceUpFullState}[5]{%
	{\tensor{j\big(\States{#1}{#2}{#3}{#4}\big)}{^{{\FieldIndices{#3}{#5}}}}}%
}
\newrobustcmd{\FieldDownState}[5]{%
	{\tensor{\zeta\big(\States{#1}{#2}{#3}{#4}\big)}{_{\ParallelFieldIndices{#1}{#2}{#5}}}}%
}
\newrobustcmd{\FieldDownFullState}[5]{%
	{\tensor{\zeta\big(\States{#1}{#2}{#3}{#4}\big)}{_{\FieldIndices{#3}{#5}}}}%
}
\newrobustcmd{\FieldDownFullStateExample}[5]{%
	{\tensor{\zeta\big(\States{#1}{#2}{#3}{#4}\big)}{_{{#5}}}}%
}
\newrobustcmd{\WaveOperatorInverseTensorUpDown}[4]{%
	{\tensor{\left(\mathcal{O}^{-1}\right)}{^{{\FieldIndices{#1}{#3}}}_{\FieldIndices{#2}{#4}}}}%
}
\newrobustcmd{\WaveOperatorTensorUpDown}[4]{%
	{\tensor{\mathcal{O}}{^{{\FieldIndices{#1}{#3}}}_{\FieldIndices{#2}{#4}}}}%
}
\newrobustcmd{\WaveOperatorTensorDownUp}[4]{%
	{\tensor{\mathcal{O}}{_{{\FieldIndices{#1}{#3}}}^{\FieldIndices{#2}{#4}}}}%
}
\newrobustcmd{\WaveOperatorTensorUpUp}[4]{%
	{\tensor{\mathcal{O}}{^{{\FieldIndices{#1}{#3}}}^{\FieldIndices{#2}{#4}}}}%
}
\newrobustcmd{\VolumeForm}[1]{%
	{\tensor{\mathcal{E}}{#1}}%
}
\newrobustcmd{\NormalisationPV}[1]{%
	{q_{#1}}%
}
\newrobustcmd{\Normalisation}[4]{%
	{c\big(\States{#1}{#2}{#3}{#4}\big)}%
}
\newrobustcmd{\PVSPODownUp}[9]{%
	{\tensor{%
	\mathcal{P}%
	\big(\States{#1}{#2}{#4}{#6},\States{#1}{#3}{#5}{#7}\big)%
	}{_{\FieldIndices{#4}{#8}}^{{\FieldIndices{#5}{#9}}}}}%
}
\newrobustcmd{\SPODownUp}[8]{%
	{\tensor{%
	\mathcal{P}%
	\big(\States{#1}{#2}{#3}{#5},\States{#1}{#2}{#4}{#6}\big)%
	}{_{\FieldIndices{#3}{#7}}^{{\FieldIndices{#4}{#8}}}}}%
}
\newrobustcmd{\PVSPOUpDown}[9]{%
	{\tensor{%
	\mathcal{P}%
	\big(\States{#1}{#2}{#4}{#6},\States{#1}{#3}{#5}{#7}\big)%
	}{^{\FieldIndices{#4}{#8}}_{{\FieldIndices{#5}{#9}}}}}%
}
\newrobustcmd{\SPOUpDown}[8]{%
	{\tensor{%
	\mathcal{P}%
	\big(\States{#1}{#2}{#3}{#5},\States{#1}{#2}{#4}{#6}\big)%
	}{^{{\FieldIndices{#3}{#7}}}_{\FieldIndices{#4}{#8}}}}%
}
\newrobustcmd{\ReducedSPODownUp}[6]{%
	{\tensor{%
	\mathcal{P}%
	\big(\States{#1}{#2}{#3}{#4}\big)%
	}{_{\ParallelFieldIndices{#1}{#2}{#5}}^{{\FieldIndices{#3}{#6}}}}}%
}
\newrobustcmd{\ReducedSPODownUpGeneral}[6]{%
	{\tensor{%
	\mathcal{P}%
	\big(\States{#1}{#2}{#3}{#4}\big)%
	}{_{{{#5}}}^{{\FieldIndices{#3}{#6}}}}}%
}
\newrobustcmd{\ReducedSPOUpDown}[6]{%
	{\tensor{%
	{\mathcal{P}%
	\big({\States{#1}{#2}{#3}{#4}}\big)}%
	}{^{{\ParallelFieldIndices{#1}{#2}{#5}}}_{{\FieldIndices{#3}{#6}}}}}%
}
\newrobustcmd{\ReducedSPOUpDownGeneral}[6]{%
	{\tensor{%
	{\mathcal{P}%
	\big({\States{#1}{#2}{#3}{#4}}\big)}%
	}{^{{{#5}}}_{{\FieldIndices{#3}{#6}}}}}%
}
\newrobustcmd{\GaugeVarying}[3]{%
	{\tensor*{g}{_{#3_{{#1^#2}}}}}%
}
\newrobustcmd{\GaugeVaryingConj}[3]{%
	{\tensor*{g}{^*_{#3_{{#1^#2}}}}}%
}
\newrobustcmd{\GaugeFixing}[3]{%
	{\tensor*{h}{_{#3_{{#1^#2}}}}}%
}
\newrobustcmd{\Mass}[3]{%
	{\tensor*{M}{_{#3_{{#1^#2}}}}}%
}
\newrobustcmd{\PVSquareMass}[2]{%
	{\tensor*{M}{^2_{#2_{{#1}}}}}%
}
\newrobustcmd{\SquareMass}[3]{%
	{\tensor*{M}{^2_{#3_{{#1^#2}}}}}%
}
\newrobustcmd{\NullVectors}[3]{%
	{#3_{{#1^#2}}}%
}
\newrobustcmd{\NullVectorsPV}[2]{%
	{#2_{{#1}}}%
}
\newrobustcmd{\NullVector}[3]{%
	{\tensor*{\mathsf{v}}{_{#3_{{#1^#2}}}}}%
}
\newrobustcmd{\RightNullVectorPV}[2]{%
	{\tensor*{\mathsf{v}}{_{#2_{{#1}}}}}%
}
\newrobustcmd{\LeftNullVectorPV}[2]{%
	{\tensor*{\mathsf{u}}{_{#2_{{#1}}}}}%
}
\newrobustcmd{\NullVectorComponents}[5]{%
	{\tensor{{\left[{\NullVector{#1}{#2}{#3}}\right]}}{_{{\States{#1}{#2}{#4}{#5}}}}}%
}
\newrobustcmd{\ConstraintNullVector}[1]{%
	{\tensor*{\mathsf{v}}{_{#1}}}%
}
\newrobustcmd{\ConstraintNullVectorConj}[1]{%
	{\tensor*{\mathsf{v}}{^\dagger_{#1}}}%
}
\newrobustcmd{\ReducedEigenVector}[1]{%
	{\tensor*{\mathsf{u}}{_{#1}}}%
}
\newrobustcmd{\ReducedEigenVectorConj}[1]{%
	{\tensor*{\mathsf{u}}{^\dagger_{#1}}}%
}
\newrobustcmd{\ReducedEigenValue}[1]{%
	{\tensor*{\lambda}{_{#1}}}%
}
\newrobustcmd{\Alpha}[1]{%
	{\tensor*{\alpha}{_{#1}}}%
}
\newrobustcmd{\Poly}[3]{%
	{\tensor*{\mathscr{#1}}{^{({#2},{#3})}}}%
}
\newrobustcmd{\MPoly}[3]{%
	{\tensor*{\mathsf{#1}}{^{({#2},{#3})}}}%
}
\newrobustcmd{\VPoly}[4]{%
	{\tensor*{\mathsf{#1}}{^{({#2},{#3})}_{#4}}}%
}
\newrobustcmd{\VPolyTranspose}[4]{%
	{\tensor*{\mathsf{#1}}{^{({#2},{#3})}_{#4}^{\ \text{T}}}}%
}
\newrobustcmd{\EigenPoly}[4]{%
	{\tensor*{{#1}}{^{({#2},{#3})}_{#4}}}%
}
\newrobustcmd{\MDZero}{%
	{\mathsf{r}}
}
\newrobustcmd{\MDTwo}{%
	{\mathsf{t}}
}
\newrobustcmd{\ReducedSource}{%
	{\tensor*{\mathsf{K}}{}}%
}
\newrobustcmd{\ReducedSourceConj}{%
	{\tensor*{\mathsf{K}}{^\dagger}}%
}
\newrobustcmd{\ReducedPropagator}{%
	{\mathsf{\Pi}}%
}
\newrobustcmd{\SpinMin}{%
	{J_{\mathrm{F}}}%
}
\newrobustcmd{\SpinMax}{%
	{J_{\mathrm{L}}}%
}
\newrobustcmd{\ParityMin}{%
	{P_{\mathrm{F}}}%
}
\newrobustcmd{\ParityMax}{%
	{P_{\mathrm{L}}}%
}
\newrobustcmd{\FieldMin}{%
	{X_{\mathrm{F}}}%
}
\newrobustcmd{\FieldMax}{%
	{X_{\mathrm{L}}}%
}
\newrobustcmd{\VectorMin}{%
	{a_{\mathrm{F}}}%
}
\newrobustcmd{\VectorMax}{%
	{a_{\mathrm{L}}}%
}
\newrobustcmd{\ZeroVector}{%
	{\mathsf{0}}%
}
\newrobustcmd{\ConstraintMatrix}{%
	{\mathsf{V}}%
}
\newrobustcmd{\SourceVector}{%
	{\mathsf{J}}%
}
\newrobustcmd{\NullVectorConj}[3]{%
	{\tensor*{\mathsf{v}}{^\dagger_{#3_{{#1^#2}}}}}%
}
\newrobustcmd{\RightNullVectorPVConj}[2]{%
	{\tensor*{\mathsf{v}}{^\dagger_{#2_{{#1}}}}}%
}
\newrobustcmd{\LeftNullVectorPVConj}[2]{%
	{\tensor*{\mathsf{u}}{^\dagger_{#2_{{#1}}}}}%
}
\newrobustcmd{\WaveOperator}{%
	{\tensor{\mathsf{O}}{}}%
}
\newrobustcmd{\WaveOperatorConj}{%
	{\tensor{\mathsf{O}}{^\ddagger}}%
}
\newrobustcmd{\WaveOperatorInverse}{%
	{\tensor{\mathsf{O}}{^{-1}}}%
}
\newrobustcmd{\MoorePenrose}{%
	{\tensor{\mathsf{O}}{^+}}%
}
\newrobustcmd{\MoorePenroseJP}[2]{%
	{\tensor*{\mathsf{O}}{^+_{{#1^#2}}}}%
}
\newrobustcmd{\MoorePenroseSJ}[2]{%
	{\tensor*{\mathsf{O}}{^+_{{#1_#2}}}}%
}
\newrobustcmd{\MoorePenroseSJPP}[2]{%
	{\tensor*{\mathsf{O}}{^+_{{#1_{#2^+}}}}}%
}
\newrobustcmd{\MoorePenroseSJPM}[2]{%
	{\tensor*{\mathsf{O}}{^+_{{#1_{#2^\pm}}}}}%
}
\newrobustcmd{\MoorePenroseSJMP}[2]{%
	{\tensor*{\mathsf{O}}{^+_{{#1_{#2^\mp}}}}}%
}
\newrobustcmd{\MoorePenroseSJMM}[2]{%
	{\tensor*{\mathsf{O}}{^+_{{#1_{#2^-}}}}}%
}


\newrobustcmd{\MoorePenroseJPP}[1]{%
	{\tensor*{\mathsf{O}}{^+_{{{#1^+}}}}}%
}
\newrobustcmd{\MoorePenroseJPM}[1]{%
	{\tensor*{\mathsf{O}}{^+_{{{#1^\pm}}}}}%
}
\newrobustcmd{\MoorePenroseJMP}[1]{%
	{\tensor*{\mathsf{O}}{^+_{{{#1^\mp}}}}}%
}
\newrobustcmd{\MoorePenroseJMM}[1]{%
	{\tensor*{\mathsf{O}}{^+_{{{#1^-}}}}}%
}
\newrobustcmd{\MoorePenroseJ}[1]{%
	{\tensor*{\mathsf{O}}{^+_{{#1}}}}%
}
\newrobustcmd{\HermitianMoorePenroseJ}[1]{%
	{\tensor*{\bar{\mathsf{O}}}{^+_{{#1}}}}%
}
\newrobustcmd{\ResHermitianMoorePenroseJ}[2]{%
	{\tensor*{\bar{\mathsf{O}}}{^+_{{#1_#2}}}}%
}
\newrobustcmd{\WaveOperatorJPP}[1]{%
	{\tensor*{\mathsf{O}}{_{{#1}^{+}}}}%
}
\newrobustcmd{\WaveOperatorJPM}[1]{%
	{\tensor*{\mathsf{O}}{_{{#1}^{\pm}}}}%
}
\newrobustcmd{\WaveOperatorJMP}[1]{%h
	{\tensor*{\mathsf{O}}{_{{#1}^{\mp}}}}%
}
\newrobustcmd{\WaveOperatorJMM}[1]{%h
	{\tensor*{\mathsf{O}}{_{{#1}^{-}}}}%
}
\newrobustcmd{\WaveOperatorJP}[2]{%
	{\tensor*{\mathsf{O}}{_{{#1}^{#2}}}}%
}
\newrobustcmd{\WaveOperatorJ}[1]{%
	{\tensor*{\mathsf{O}}{_{{#1}}}}%
}
\newrobustcmd{\ReducedWaveOperatorJ}[1]{%
	{\tensor*{\mathsf{o}}{_{{#1}}}}%
}
\newrobustcmd{\ReducedWaveOperatorRotatedJ}[1]{%
	{\tensor*{\tilde{\mathsf{o}}}{_{{#1}}}}%
}
\newrobustcmd{\WaveOperatorJConj}[1]{%
	{\tensor*{\mathsf{O}}{_{{#1}}^\ddagger}}%
}
\newrobustcmd{\WaveOperatorJPComponents}[6]{%
	{\tensor{\left[\WaveOperatorJP{#1}{#2}\right]}{_{\States{#1}{#2}{#3}{#5}\States{#1}{#2}{#4}{#6}}}}%
}
\newrobustcmd{\WaveOperatorJComponents}[7]{%
	{\tensor{\left[\WaveOperatorJ{#1}\right]}{_{\States{#1}{#2}{#4}{#6}\States{#1}{#3}{#5}{#7}}}}%
}
\newrobustcmd{\Propagator}{%
	{\tensor{\mathsf{P}}{}}%
}
\newrobustcmd{\PropagatorJ}[1]{%
	{\tensor{\mathsf{\Pi}}{_{#1}}}%
}
\newrobustcmd{\Similarity}{%
	{\tensor{\mathsf{U}}{}}%
}
\newrobustcmd{\SimilarityJ}[1]{%
	{\tensor{\mathsf{U}}{_#1}}%
}
\newrobustcmd{\VimilarityJ}[1]{%
	{\tensor{\mathsf{V}}{_#1}}%
}
\newrobustcmd{\WaveOperatorFullJ}[1]{%
	{\tensor{\mathsf{\Omega}}{_#1}}%
}
\newrobustcmd{\WaveOperatorFullJInv}[1]{%
	{\tensor*{\mathsf{\Omega}}{_#1^{-1}}}%
}
\newrobustcmd{\ResWaveOperatorFullJInv}[2]{%
	{\tensor*{\mathsf{\Omega}}{_{#1_#2}^{-1}}}%
}
\newrobustcmd{\Source}{%
	{\tensor{\mathsf{j}}{}}%
}
\newrobustcmd{\SourceConj}{%
	{\tensor{\mathsf{j}}{^\dagger}}%
}
\newrobustcmd{\Field}{%
	{\tensor{\upzeta}{}}%
}
\newrobustcmd{\FieldConj}{%
	{\tensor{\upzeta}{^\dagger}}%
}
\newrobustcmd{\Powers}[3]{%
	{#3_{{#1^#2}}}%
}
\newrobustcmd{\PartialEigenvalue}[2]{%
	{\lambda_{{#1_#2}}}%
}
\newrobustcmd{\PartialEigenvalueBoth}[3]{%
	{\lambda_{{#1_{#2^#1}}}}%
}
\newrobustcmd{\TotalEigenvector}[5]{%
	{\tensor*{\mathsf{V}}{_{{#1}_{{#2}}}}\big(\States{#2}{#3}{#4}{#5}\big)}%
}
\newrobustcmd{\TotalEigenvectorConj}[5]{%
	{\tensor*{\mathsf{V}}{_{{#1}_{{#2}}}^\ddagger}\big(\States{#2}{#3}{#4}{#5}\big)}%
}
\newrobustcmd{\Eigenvector}[2]{%
	{\tensor*{\mathsf{v}}{_{{#1}_{{#2}}}}}%
}
\newrobustcmd{\PartialEigenvector}[3]{%
	{\tensor*{\mathsf{v}}{_{{#1}_{{#2^#3}}}}}%
}
\newrobustcmd{\PartialEigenvectorConj}[3]{%
	{\tensor*{\mathsf{v}}{^\dagger_{{#1}_{{#2^#3}}}}}%
}
\newrobustcmd{\EigenvectorConj}[2]{%
	{\tensor*{\mathsf{v}}{^\dagger_{{#1}_{{#2}}}}}%
}
\newrobustcmd{\PartialSourceMatrix}[1]{%
	{\tensor*{\mathsf{J}}{_{#1}}}%
}
\newrobustcmd{\LimitPartialSourceMatrix}[2]{%
	{\tensor*{\mathsf{J}}{_{{#1}_{#2}}}}%
}
\newrobustcmd{\ConstrainedPartialSourceMatrix}[1]{%
	{\tensor*{\bar{\mathsf{J}}}{_{#1}}}%
}
\newrobustcmd{\LimitConstrainedPartialSourceMatrix}[2]{%
	{\tensor*{\bar{\mathsf{J}}}{_{{#1}_{#2}}}}%
}
\newrobustcmd{\PartialSource}[2]{%
	{\tensor*{\mathsf{J}}{_{{#1^#2}}}}%
}
\newrobustcmd{\PartialSourceConj}[2]{%
	{\tensor*{\mathsf{J}}{^\dagger_{{#1^#2}}}}%
}
\newrobustcmd{\PVMasses}[2]{%
	{#2_{{#1}}}%
}
\newrobustcmd{\Masses}[3]{%
	{#3_{{#1^#2}}}%
}
\newrobustcmd{\NewRes}[2]{%
	{\ \mathop{\mathrm{Res}}_{#1\mapsto#2}}%
}
\newrobustcmd{\NewLim}[2]{%
	{\ \mathop{\mathrm{Lim}}_{#1\mapsto#2}}%
}
\newrobustcmd{\AMat}[1]{%
	{\mathsf{A}}%
}
\newrobustcmd{\AMatT}[1]{%
	{\mathsf{A}}^{\text{T}}%
}
\newrobustcmd{\AMatU}[1]{%
	\tensor[^{\text{s}}]{\mathsf{A}}{}%
}
\newrobustcmd{\AMatUt}[1]{%
	\tensor[^{\text{s}}]{\tilde{\mathsf{A}}}{}%
}
\newrobustcmd{\AMatO}[1]{%
	\tensor[^{\text{a}}]{\mathsf{A}}{}%
}
\newrobustcmd{\BMat}[1]{%
	{\mathsf{B}}%
}
\newrobustcmd{\BMatT}[1]{%
	{\mathsf{B}}^{\text{T}}%
}
\newrobustcmd{\BMatU}[1]{%
	\tensor[^{\text{s}}]{\mathsf{B}}{}%
}
\newrobustcmd{\BMatO}[1]{%
	\tensor[^{\text{a}}]{\mathsf{B}}{}%
}
\newrobustcmd{\BMatOt}[1]{%
	\tensor[^{\text{a}}]{\tilde{\mathsf{B}}}{}%
}
\newrobustcmd{\CMat}[1]{%
	{\mathsf{C}}%
}
\newrobustcmd{\CMatT}[1]{%
	{\mathsf{C}}^{\text{T}}%
}
\newrobustcmd{\CMatU}[1]{%
	\tensor[^{\text{s}}]{\mathsf{C}}{}%
}
\newrobustcmd{\CMatUt}[1]{%
	\tensor[^{\text{s}}]{\tilde{\mathsf{C}}}{}%
}
\newrobustcmd{\HigherSpinField}[1]{%
  \tensor{h}{#1}
}
\newrobustcmd{\HigherSpinSource}[1]{%
  \tensor{F}{#1}
}
\newrobustcmd{\ECT}[1]{%
	\tensor{\mathscr{T}}{#1}
}
\newrobustcmd{\ECR}[1]{%
	\tensor{\mathscr{R}}{#1}
}
\newrobustcmd{\Holst}[1]{%
\tensor{\tilde{\mathscr{R}}}{#1}
}
\newrobustcmd{\MAGQ}[1]{%
	\tensor{\mathcal{Q}}{#1}
}
\newrobustcmd{\MAGQt}[1]{%
	\tensor{\tilde{\mathcal{Q}}}{#1}
}
\newrobustcmd{\B}[1]{%
	\tensor{\mathcal{B}}{#1}%
}
\newrobustcmd{\VectorField}[1]{%
	\tensor{\mathcal{A}}{#1}%
}
\newrobustcmd{\TwoFormField}[1]{%
	\tensor{\mathcal{B}}{#1}%
}
\newrobustcmd{\GaugePotential}[1]{%
	\tensor{\xi}{#1}%
}
\newrobustcmd{\ThreeFormField}[1]{%
	\tensor{\mathcal{C}}{#1}%
}
\newrobustcmd{\PForm}[1]{%
	\tensor{\vphantom{l^{l^2}}\smash{\stackrel{\raisebox{-3pt}{\scalebox{0.55}{$({#1})$}}}{\scalebox{0.75}{$\mathcal{B}$}}}}{}%
}
\newrobustcmd{\PFormSource}[1]{%
	\tensor{\vphantom{l^{l^2}}\smash{\stackrel{\raisebox{-3pt}{\scalebox{0.55}{$({#1})$}}}{\scalebox{0.75}{$\mathcal{J}$}}}}{}%
}
\newrobustcmd{\DForm}[1]{%
	\tensor{dx}{#1}%
}
\newrobustcmd{\CT}[1]{%
	\tensor{{c^\text{T}}}{#1}%
}
\newrobustcmd{\dCT}[1]{%
	\tensor{{\dot{c}^\text{T}}}{#1}%
}
\newrobustcmd{\tCT}[1]{%
	\tensor{{\tilde{c}^\text{T}}}{#1}%
}
\newrobustcmd{\tBT}[1]{%
	\tensor{{\tilde{b}^\text{T}}}{#1}%
}
\newrobustcmd{\dBT}[1]{%
	\tensor{{\dot{b}^\text{T}}}{#1}%
}
\newrobustcmd{\BT}[1]{%
	\tensor{{b^\text{T}}}{#1}%
}
\newrobustcmd{\dB}[1]{%
	\tensor{\dot{\mathcal{B}}}{#1}%
}
\newrobustcmd{\A}[1]{%
	\tensor{\mathcal{A}}{#1}%
}
\newrobustcmd{\J}[1]{%
	\tensor{\mathcal{J}}{#1}%
}
\newrobustcmd{\JForm}[2]{%
	\tensor{\mathcal{J}}{_{(\mathcal{#1})}#2}%
}
\newrobustcmd{\dJ}[1]{%
	\tensor{\dot{\mathcal{J}}}{#1}%
}
\newrobustcmd{\BConj}[1]{%
	\tensor{{B^\dagger}}{#1}%
}
\newrobustcmd{\N}[1]{%
	\tensor{n}{#1}%
}
\newrobustcmd{\Eps}[1]{%
	\tensor{\varepsilon}{#1}%
}
\newrobustcmd{\En}[1]{%
	\mathcal{E}%
}
\newrobustcmd{\Mo}[1]{%
	p%
}
\newrobustcmd{\JConj}[1]{%
	\tensor{{J^\dagger}}{#1}%
}
\newrobustcmd{\K}[1]{%
	\tensor{K}{_#1}%
}
\newrobustcmd{\KConj}[1]{%
	\tensor*{{K^{\dagger}}}{_{#1}}%
}
%general linear group in four real dimensions
\newrobustcmd{\glfourr}{%
  {\mathrm{GL}(4,\mathbb{R})}%
}
%special linear group in two complex dimensions
\newrobustcmd{\sltwoc}{%
  {\mathrm{SL}(2,\mathbb{C})}%
}
%poincare group
\newrobustcmd{\poincare}{%
  {\mathbb{R}^{1,3}\rtimes\mathrm{SO}^+(1,3)}%
}
%poincare group formal
\newrobustcmd{\poincaref}{%
  {\mathrm{P}(1,3)}%
}
%weyl group
\newrobustcmd{\weyl}{%
  {\mathrm{W}(1,3)}%
}
%weyl group
\newrobustcmd{\conformal}{%
  {\mathrm{C}(1,3)}%
}
%diffeomorphism group
\newrobustcmd{\diffeomorphism}{%
  {\mathbb{R}^{1,3}}%
}
%lorentz group
\newrobustcmd{\soonethree}{%
  {\mathrm{SO}^+(1,3)}%
}
%special orthogonal group
\newrobustcmd{\othree}{%
  {\mathrm{SO}(3)}%
}
%special orthogonal group
\newrobustcmd{\sothree}{%
  {\mathrm{SO}(3)}%
}
%special orthogonal group
\newrobustcmd{\sotwo}{%
  {\mathrm{SO}(2)}%
}
%QCD group
\newrobustcmd{\suthreec}{%
  {\mathrm{SU}(3)_{\text{c}}}%
}
%weak isospin group
\newrobustcmd{\sutwol}{%
  {\mathrm{SU}(2)_{\text{L}}}%
}
%weak hypercharge group
\newrobustcmd{\uoney}{%
  {\mathrm{U}(1)_{\text{Y}}}%
}
%weak hypercharge group
\newrobustcmd{\uone}{%
  {\mathrm{U}(1)}%
}
%electromagnetic group
\newrobustcmd{\uoneem}{%
  {\mathrm{U}(1)_{\text{em}}}%
}
\newrobustcmd{\sutwo}{%
  {\mathrm{SU}(2)}%
}
\newrobustcmd{\Planck}{%
	{M_{\text{Pl}}}%
}
\newrobustcmd{\ovl}[1]{%
	\overline{#1}%
}
\newrobustcmd{\FieldG}[1]{%
	\tensor{g}{#1}
}
\newrobustcmd{\Hermitian}{%
	\mathsf{H}%	
}
\newrobustcmd{\HermitianMP}{%
	\tensor*{\mathsf{H}}{^+}%	
}
\newrobustcmd{\SkewHermitian}{%
	\mathsf{A}%	
}
\newrobustcmd{\ChequerHermitian}{%
	{\mathsf{C}}%
}
\newrobustcmd{\ChequerHermitianConj}{%
	{\tensor{\mathsf{C}}{^\ddagger}}%	
}
\newrobustcmd{\ChequerHermitianMP}{%
	\tensor{\mathsf{C}}{^+}%	
}
\newrobustcmd{\General}{%
	\mathsf{M}%	
}
\newrobustcmd{\GeneralConj}{%
	\tensor{\mathsf{M}}{^\ddagger}%	
}
\newrobustcmd{\GeneralMP}{%
	\tensor{\mathsf{M}}{^+}%	
}
\newrobustcmd{\HermitianDiagonal}{%
	\tensor*{\mathsf{C}}{_{dh}}%	
}
\newrobustcmd{\HermitianDiagonalConj}{%
	\tensor*{\mathsf{C}}{_{dh}^\dagger}%	
}
\newrobustcmd{\SkewHermitianOffDiagonal}{%
	\tensor*{\mathsf{C}}{_{os}}%	
}
\newrobustcmd{\SkewHermitianOffDiagonalConj}{%
	\tensor*{\mathsf{C}}{_{os}^\dagger}%	
}

\newrobustcmd{\InverseHermitianDiagonal}{%
	\tensor*{\mathsf{C}}{_{dh}^{-1}}%	
}
\newrobustcmd{\InverseHermitianDiagonalConj}{%
	\tensor*{\mathsf{C}}{_{dh}^{-1}^\dagger}%	
}
\newrobustcmd{\InverseHermitianOffDiagonal}{%
	\tensor*{\mathsf{C}}{_{oh}^{-1}}%	
}
\newrobustcmd{\InverseHermitianOffDiagonalConj}{%
	\tensor*{\mathsf{C}}{_{oh}^{-1}^\dagger}%	
}
\newrobustcmd{\InverseSkewHermitianOffDiagonal}{%
	\tensor*{\mathsf{C}}{_{os}^{-1}}%	
}
\newrobustcmd{\InverseSkewHermitianOffDiagonalConj}{%
	\tensor*{\mathsf{C}}{_{os}^{-1}^\dagger}%	
}
\newrobustcmd{\InverseSkewHermitianDiagonal}{%
	\tensor*{\mathsf{C}}{_{ds}^{-1}}%	
}
\newrobustcmd{\InverseSkewHermitianDiagonalConj}{%
	\tensor*{\mathsf{s}}{_{+}^\dagger}%	
}
\newrobustcmd{\Ca}{%
	{\tensor*{\mathsf{C}}{_{+}}}%	
}
\newrobustcmd{\CaConj}{%
	{\tensor*{\mathsf{C}}{_{+}^\dagger}}%	
}
\newrobustcmd{\Cb}{%
	\tensor*{\mathsf{C}}{_{\pm}}%	
}
\newrobustcmd{\CbConj}{%
	\tensor*{\mathsf{C}}{_{\pm}^\dagger}%	
}
\newrobustcmd{\Cc}{%
	\tensor*{\mathsf{C}}{_{\mp}}%	
}
\newrobustcmd{\CcConj}{%
	\tensor*{\mathsf{C}}{_{\mp}^\dagger}%	
}
\newrobustcmd{\Cd}{%
	\tensor*{\mathsf{C}}{_{-}}%	
}
\newrobustcmd{\CdConj}{%
	\tensor*{\mathsf{C}}{_{-}^\dagger}%	
}
\newrobustcmd{\MCa}{%
	\tensor*{\mathsf{M}}{_{+}}%	
}
\newrobustcmd{\MCaConj}{%
	\tensor*{\mathsf{M}}{_{+}^\dagger}%	
}
\newrobustcmd{\MCb}{%
	\tensor*{\mathsf{M}}{_{\pm}}%	
}
\newrobustcmd{\MCbConj}{%
	\tensor*{\mathsf{M}}{_{\pm}^\dagger}%	
}
\newrobustcmd{\MCc}{%
	\tensor*{\mathsf{M}}{_{\mp}}%	
}
\newrobustcmd{\MCcConj}{%
	\tensor*{\mathsf{M}}{_{\mp}^\dagger}%	
}
\newrobustcmd{\MCd}{%
	\tensor*{\mathsf{M}}{_{-}}%	
}
\newrobustcmd{\MCdConj}{%
	\tensor*{\mathsf{M}}{_{-}^\dagger}%	
}
\newrobustcmd{\RightNullVector}[1]{%
	{\tensor*{\mathsf{v}}{_{#1}}}%
}
\newrobustcmd{\RightNullVectorConj}[1]{%
	{\tensor*{\mathsf{v}}{_{#1}^\dagger}}%
}
\newrobustcmd{\LeftNullVector}[1]{%
	{\tensor*{\mathsf{u}}{_{#1}}}%
}
\newrobustcmd{\LeftNullVectorConj}[1]{%
	{\tensor*{\mathsf{u}}{_{#1}^\dagger}}%
}
\newrobustcmd{\PlusNullVector}[1]{%
	{\tensor*{\mathsf{v}}{_{{#1}+}}}%
}
\newrobustcmd{\PlusNullVectorConj}[1]{%
	{\tensor*{\mathsf{v}}{_{{#1}+}^\dagger}}%
}
\newrobustcmd{\MinusNullVector}[1]{%
	{\tensor*{\mathsf{v}}{_{{#1}-}}}%
}
\newrobustcmd{\MinusNullVectorConj}[1]{%
	{\tensor*{\mathsf{v}}{_{{#1}-}^\dagger}}%
}
\newrobustcmd{\WaveOperatorRotatedJVV}[1]{%
	{\tensor*{\tilde{\mathsf{o}}}{_{{#1_{\text{m}}}}}}%
}
\newrobustcmd{\WaveOperatorJVV}[1]{%
	{\tensor*{\mathsf{o}}{_{{#1_{\text{m}}}}}}%
}
\newrobustcmd{\WaveOperatorJVL}[1]{%
	{\tensor*{\mathsf{o}}{_{{#1_{\text{m}\gamma}}}}}%
}
\newrobustcmd{\WaveOperatorJLV}[1]{%
	{\tensor*{\mathsf{o}}{_{{#1_{\gamma\text{m}}}}}}%
}
\newrobustcmd{\WaveOperatorJLL}[1]{%
	{\tensor*{\mathsf{o}}{_{{#1_{\gamma}}}}}%
}
\newrobustcmd{\Kinetic}[1]{%
	{\tensor*{\mathsf{g}}{#1}}%
}
\newrobustcmd{\NewKinetic}[1]{%
	{\tensor*{\tilde{\mathsf{g}}}{#1}}%
}
\newrobustcmd{\KineticJ}[1]{%
	{\tensor*{\mathsf{K}}{_{#1}}}%
}
\newrobustcmd{\KineticInverseJ}[1]{%
	{\tensor*{\mathsf{K}}{^{+}_{#1}}}%
}
\newrobustcmd{\MassJ}[1]{%
	{\tensor*{\mathsf{M}}{_{#1}}}%
}
\newrobustcmd{\PostMassJ}[1]{%
	{\tensor*{\mathsf{L}}{_{#1}}}%
}
\newrobustcmd{\WaveOperatorJVVInverse}[1]{%
	{\tensor*{\mathsf{o}}{^{+}_{{#1_{\text{m}}}}}}%
}
\newrobustcmd{\WaveOperatorJVLInverse}[1]{%
	{\tensor*{\mathsf{o}}{^{+}_{{#1_{\text{m}\gamma}}}}}%
}
\newrobustcmd{\WaveOperatorJLVInverse}[1]{%
	{\tensor*{\mathsf{o}}{^{+}_{{#1_{\gamma\text{m}}}}}}%
}
\newrobustcmd{\WaveOperatorJLLInverse}[1]{%
	{\tensor*{\mathsf{o}}{^{+}_{{#1_{\gamma}}}}}%
}
\newrobustcmd{\NormalMatrix}[4]{%
	\left[\ 
		\begin{tblr}{colspec=cc}
			 {#1} &  {#2}\\
			 {#3} &  {#4}
		\end{tblr}
	\ \right]
}
\newrobustcmd{\Chequer}[4]{%
	\left[\ 
		\begin{tblr}{colspec=cc}
			\SetCell{bg=gray!10} \vphantom{X^\ddagger_i}{#1} & \SetCell{bg=gray!40} {#2}\\
			\SetCell{bg=gray!40} \vphantom{X^\ddagger_i}{#3} & \SetCell{bg=gray!10} {#4}
		\end{tblr}
	\ \right]
}
\newrobustcmd{\ChequerMain}[4]{%
	\left[\ 
		\begin{tblr}{colspec=cc}
			\SetCell{bg=gray!10} \vphantom{X^\ddagger_i}{#1} & \SetCell{bg=gray!10} {#2}\\
			\SetCell{bg=gray!10} \vphantom{X^\ddagger_i}{#3} & \SetCell{bg=gray!10} {#4}
		\end{tblr}
	\ \right]
}
\newrobustcmd{\ChequerVectorConj}[2]{%
	\left[\ 
		\begin{tblr}{colspec=cc}
			\SetCell{bg=gray!10} \vphantom{X^\ddagger_i}{#1} & \SetCell{bg=gray!40} {#2}
		\end{tblr}
	\ \right]
}
\newrobustcmd{\ChequerVector}[2]{%
	\left[\ 
		\begin{tblr}{colspec=c}
			\SetCell{bg=gray!10} \vphantom{X^\ddagger_i}{#1} \\
			\SetCell{bg=gray!40} \vphantom{X^\ddagger_i}{#2} 
		\end{tblr}
	\ \right]
}
\newrobustcmd{\MAGA}[1]{%
  \tensor{A}{#1}
}
\newrobustcmd{\MAGF}[1]{%
    \tensor{\mathcal{F}}{#1}
}
\newrobustcmd{\MAGHolst}[1]{%
	\tensor{\tilde{\mathcal{F}}}{#1}
}
\newrobustcmd{\MAGT}[1]{%
    \tensor{\mathcal{T}}{#1}
}
\newrobustcmd{\MAGD}[1]{%
	\tensor{\mathcal{D}}{#1}
}
\newrobustcmd{\Con}[1]{%
    \tensor{\Gamma}{#1}%
}
\newrobustcmd{\MAGg}[1]{%
    \tensor{g}{#1}%
}
\newrobustcmd{\PD}[1]{%
    \tensor{\partial}{#1}%
}

